Provenance-based Data Skipping (TechReport)

Database systems analyze queries to determine upfront which data is needed for answering them and use indexes and other physical design techniques to speed-up access to that data. However, for important classes of queries, e.g., HAVING and top-k queries, it is impossible to determine up-front what data is relevant. To overcome this limitation, we develop provenance-based data skipping (PBDS), a novel approach that generates provenance sketches to concisely encode what data is relevant for a query. Once a provenance sketch has been captured it is used to speed up subsequent queries. PBDS can exploit physical design artifacts such as indexes and zone maps. Our approach significantly improves performance for both disk-based and main-memory database systems.

==> lstdefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{lstpurple}{rgb}{0.5,0,0.5}
\definecolor{lstred}{rgb}{1,0,0}
\definecolor{lstreddark}{rgb}{0.7,0,0}
\definecolor{lstredl}{rgb}{0.64,0.08,0.08}
\definecolor{lstmildblue}{rgb}{0.66,0.72,0.78}
\definecolor{lstblue}{rgb}{0,0,1}
\definecolor{lstmildgreen}{rgb}{0.42,0.53,0.39}
\definecolor{lstgreen}{rgb}{0,0.5,0}
\definecolor{lstorangedark}{rgb}{0.6,0.3,0}
\definecolor{lstorange}{rgb}{0.75,0.52,0.005}
\definecolor{lstorangelight}{rgb}{0.89,0.81,0.67}
\definecolor{lstbeige}{rgb}{0.90,0.86,0.45}


% Declare bold typewriter font with Computer Modern
\DeclareFontShape{OT1}{cmtt}{bx}{n}{<5><6><7><8><9><10><10.95><12><14.4><17.28><20.74><24.88>cmttb10}{}

%%%%%%%%%% SQL + proveannce listing settings
\lstdefinestyle{psql}
{
tabsize=2,
basicstyle=\footnotesize\upshape\ttfamily,
language=SQL,
morekeywords={PROVENANCE,BASERELATION,INFLUENCE,COPY,ON,TRANSPROV,TRANSSQL,TRANSXML,CONTRIBUTION,COMPLETE,TRANSITIVE,NONTRANSITIVE,EXPLAIN,SQLTEXT,GRAPH,IS,ANNOT,THIS,XSLT,MAPPROV,cxpath,OF,TRANSACTION,SERIALIZABLE,COMMITTED,INSERT,INTO,WITH,SCN,UPDATED,WINDOW},
extendedchars=false,
keywordstyle=\bfseries,
mathescape=true,
escapechar=@,
sensitive=true
}


%%%%%%%%%% SQL + proveannce listing settings - colorful version
%basicstyle=\footnotesize\upshape\ttfamily,
\lstdefinestyle{psqlcolor}
{
tabsize=2,
basicstyle=\footnotesize\upshape\ttfamily,
language=SQL,
morekeywords={PROVENANCE,BASERELATION,INFLUENCE,COPY,ON,TRANSPROV,TRANSSQL,TRANSXML,CONTRIBUTION,COMPLETE,TRANSITIVE,NONTRANSITIVE,EXPLAIN,SQLTEXT,GRAPH,IS,ANNOT,THIS,XSLT,MAPPROV,cxpath,OF,TRANSACTION,SERIALIZABLE,COMMITTED,INSERT,INTO,WITH,SCN,UPDATED,FOLLOWING,RANGE,UNBOUNDED,PRECEDING,OVER,PARTITION,WINDOW},
extendedchars=false,
keywordstyle=\bfseries\color{lstpurple},
deletekeywords={count,min,max,avg,sum,lag,first_value,last_value},
keywords=[2]{count,min,max,avg,sum,lag,first_value,last_value,lead,row_number},
keywordstyle=[2]\color{lstblue},
stringstyle=\color{lstreddark},
commentstyle=\color{lstgreen},
mathescape=true,
escapechar=@,
sensitive=true
}


%%%%%%%%%% DATALOG style
\lstdefinestyle{datalog}
{
basicstyle=\footnotesize\upshape\ttfamily,
language=prolog
}




%%%%%%%%%% listings settings for pseudo code
\lstdefinestyle{pseudocode}
{
  tabsize=3,
  basicstyle=\small,
  language=c,
  morekeywords={if,else,foreach,case,return,in,or},
  extendedchars=true,
  mathescape=true,
  literate={:=}{{$\gets$}}1 {<=}{{$\leq$}}1 {!=}{{$\neq$}}1 {append}{{$\listconcat$}}1 {calP}{{$\cal P$}}{2},
  keywordstyle=\color{lstpurple},
  escapechar=&,
  numbers=left,
  numberstyle=\color{lstgreen}\small\bfseries,
  stepnumber=1,
  numbersep=5pt,
}

%%%%%%%%%% XML listings settings
\lstdefinestyle{xmlstyle}
{
  tabsize=3,
  basicstyle=\small,
  language=xml,
  extendedchars=true,
  mathescape=true,
  escapechar=£,
  tagstyle=\color{keywordpurple},
  usekeywordsintag=true,
  morekeywords={alias,name,id},
  keywordstyle=\color{lstred}
}


==> sections/beneficial_query_structure.tex <==
\section{Beneficial Query Structures}
\label{sec:typic-query-struct}

In general, our technique is effective in cases where only a fraction of the input is actually relevant for answering the query, but where it is impossible to statically determine based on the query alone what this subset is. Commonly used query types that match this description are:

Queries that filter the output of an aggregation such as top-k queries and queries with a having clause.

Return all departments with more than 100 employees.

\begin{lstlisting}
SELECT dept, count(*)
FROM employee
GROUP BY dept
HAVING count(*) > 100
\end{lstlisting}

Return the 3 largest departments.

\begin{lstlisting}
SELECT dept
FROM employee
GROUP BY dept
ORDER BY count(*) DESC
LIMIT 3
\end{lstlisting}

\begin{itemize}
\item Where would materialized views not help?
  \begin{itemize}
  \item Lower size (we only need a few bytes)
  \item We can exploit existing physical design (indexes, partitions, zone maps)
  \item Smaller search space (if we limit the options of what type of provenance to capture)
  \end{itemize}
\end{itemize}

\subsection{Query Answering with Provenance}
\label{sec:query-answering-with}

Given provenance of past queries, can we

==> sections/exp_figs_short1.tex <==
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
  \centering
   %%%%%%%%%%%%%%%%%%%% selectivity
%  \begin{minipage}{0.48\linewidth}
%    \includegraphics[width=1\linewidth,trim=0pt 5pt 0 0pt, clip]{figs/binary_search/selectivity_1g_stack.pdf}
%    \trimfigspace
%      	\caption{Selectivity of range-partition provenance sketches for the TPC-H 1GB.}
%      	\label{fig:sel-tpch-1gb}
%      \end{minipage}
%        \begin{minipage}{0.46\linewidth}
%    \begin{subfigure}{0.49\linewidth}
%      \centering
%      \includegraphics[width=1\linewidth,trim=0pt 25pt 0pt 25pt, clip]{figs/realdb/post_realdb_runtime.pdf}
%      %\trimfigspace
%      \caption{Crimes - Use (OR)}
%      \label{fig:realdb-use}
%    \end{subfigure}
%    \begin{subfigure}{0.49\linewidth}
%      \centering
%      \includegraphics[width=1\linewidth,trim=0pt 25pt 0pt 25pt, clip]{figs/realdb/post_realdb_capture.pdf}
%      %\trimfigspace
%      \caption{Crimes - Capture}
%      \label{fig:realdb-cap}
%    \end{subfigure}
%        \begin{subfigure}{0.49\linewidth}
%      \includegraphics[width=1\linewidth,trim=10pt 22pt 10pt 0pt, clip]{figs/realdb/stack_overflow_runtime.pdf}
%      \caption{SOF - Use (BS)}
%      \label{fig:stack-use}
%    \end{subfigure}
%    \begin{subfigure}{0.49\linewidth}
%      \includegraphics[width=1\linewidth,trim=10pt 22pt 10pt 0pt, clip]{figs/realdb/stack_overflow_capture.pdf}
%      \caption{SOF - Capture}
%      \label{fig:stack-cap}
%    \end{subfigure}
%    \trimfigspace
%    \caption{Real world data}
%      % Runtime and overhead of queries instrumented to capture provenance sketches relative to queries without instrumentation for real world datasets on Postgres}
%    \label{fig:real-word}
%   \end{minipage}


  %%%%%%%%%%%%%%%%%%%% PS legend
  \begin{minipage}{1.0\linewidth}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/pslegend.pdf}
  \end{minipage}

   %%%%%%%%%%%%%%%%%%%% Postgres runtime + overhead
  \begin{minipage}[t]{1.0\linewidth}
    \begin{subfigure}{0.49\linewidth}
      \centering
      \includegraphics[height=3cm,trim=25pt 25pt 0 24pt, clip]{figs/binary_search/version1/post_tpch_1GB_runtime.pdf}
      \trimfigspace
      \caption{Postgres Use - 1GB (BS)}
      \label{fig:tpch-post-1gb}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
      \centering
      \includegraphics[height=3cm,trim=25pt 25pt 0 24pt, clip]{figs/binary_search/version1/post_tpch_1GB_capture.pdf}
      \trimfigspace
      \caption{Postgres Capture - 1GB}
      \label{fig:cap-tpch-post-1gb}
    \end{subfigure}
  \end{minipage}

 %%%%%%%%%%%%%%%%%%%% postgres overhead and selectivities
  \begin{minipage}{1.0\linewidth}
    \begin{subfigure}{0.331\linewidth}
      \centering
      \includegraphics[height=3cm,trim=25pt 25pt 0 28pt, clip]{figs/binary_search/version1/post_tpch_1GB_runtime_index.pdf}
      \trimfigspace
      \caption{Runtime - Postgres - 1GB (OR)}
      \label{fig:use-tpch-post-1gb-or}
    \end{subfigure}
    \begin{subfigure}{0.331\linewidth}
      \includegraphics[height=3cm,trim=25pt 25pt 0 28pt, clip]{figs/binary_search/version1/post_tpch_10GB_runtime.pdf}
      \trimfigspace
      \caption{Postgres Use - 10GB (BS)}
      \label{fig:tpch-post-10gb}
    \end{subfigure}
    \begin{subfigure}{0.331\linewidth}
      \includegraphics[height=3cm,trim=25pt 25pt 0 28pt, clip]{figs/binary_search/version1/post_tpch_10GB_capture.pdf}
      \trimfigspace
      \caption{Postgres Capture - 10GB}
      \label{fig:cap-tpch-post-10gb}
    \end{subfigure}
  \end{minipage}

   %%%%%%%%%%%%%%%%%%%% monetdb runtime + overhead
  \begin{minipage}{1.0\linewidth}
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=1\linewidth,trim=20pt 25pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_1GB_runtime.pdf}
      \trimfigspace[-5mm]
      \caption{MonetDB Use - 1GB (OR)}
      \label{fig:monetdb-tpch-1gb}
    \end{subfigure}
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=1\linewidth,trim=20pt 25pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_10GB_runtime.pdf}
      \trimfigspace[-5mm]
      \caption{MonetDB Use - 10GB (OR)}
      \label{fig:monetdb-tpch-10gb}
    \end{subfigure}
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=1\linewidth,trim=20pt 25pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_1GB_capture.pdf}
      \trimfigspace[-5mm]
      \caption{MonetDB Capture - 1GB}
      \label{fig:monetdb-tpch-overhead-1gb}
    \end{subfigure}
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=1\linewidth,trim=20pt 25pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_10GB_capture.pdf}
      \trimfigspace[-5mm]
      \caption{MonetDB Capture - 10GB}
      \label{fig:monetdb-tpch-overhead-10gb}
    \end{subfigure}
    \trimfigspace
    \caption{Performance of provenance sketch capture and use for TPC-H queries.}
    \label{fig-exp-runtimes-usage}
  \end{minipage}


%    %%%%%%%%%%%%%%%%%%%% monetdb runtime + postgres or
%   \begin{minipage}{1.0\linewidth}
%     \begin{subfigure}{0.34\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_1GB_runtime.pdf}
%       \trimfigspace
%       \caption{Runtime - MonetDB - 1GB (BS)}
%       \label{fig:monetdb-tpch-1gb}
%     \end{subfigure}
%     \begin{subfigure}{0.34\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_10GB_runtime.pdf}
%       \trimfigspace
%       \caption{Runtime - MonetDB - 10GB (BS)}
%       \label{fig:monetdb-tpch-10gb}
%     \end{subfigure}
%     \begin{subfigure}{0.31\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/binary_search/version1/post_tpch_1GB_runtime_index.pdf}
%       \trimfigspace
%       \caption{Runtime - Postgres - 1GB (OR)}
%       \label{fig:use-tpch-post-1gb-or}
%     \end{subfigure}
% %    \caption{Runtime of queries instrumented for \pbds ~(PS) compared to no instrumentation (\nor).}
% %    \label{fig-exp-runtimes-usage}
%   \end{minipage}
%   %%%%%%%%%%%%%%%%%%%% USAGE posgres + monetdb 1g capture
%   \begin{minipage}{1.0\linewidth}
%     \begin{subfigure}{0.37\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/binary_search/version1/post_tpch_1GB_runtime.pdf}
%       \caption{Runtime - Postgres - 1GB (BS)}
%       \label{fig:tpch-post-1gb}
%     \end{subfigure}
%     \begin{subfigure}{0.31\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/binary_search/version1/post_tpch_10GB_runtime.pdf}
%       \caption{Runtime - Postgres - 10GB (BS)}
%       \label{fig:tpch-post-10gb}
%     \end{subfigure}
%     \begin{subfigure}{0.31\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_1GB_capture.pdf}
%       \caption{Overhead - MonetDB - 1GB}
%       \label{fig:monetdb-tpch-overhead-1gb}
%     \end{subfigure}
% %    \caption{Runtime of queries instrumented for \pbds ~(PS) compared to no instrumentation (\nor).}
% %    \label{fig-exp-runtimes-usage}
%   \end{minipage}
%   %%%%%%%%%%%%%%%%%%%% CAPTURE posgres + monetdb 10g capture
%   \begin{minipage}{1.0\linewidth}
%     \begin{subfigure}{0.37\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/binary_search/version1/post_tpch_1GB_capture.pdf}
%       \caption{Overhead - Postgres - 1GB}
%       \label{fig:cap-tpch-post-1gb}
%     \end{subfigure}
%     \begin{subfigure}{0.31\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/binary_search/version1/post_tpch_10GB_capture.pdf}
%       \caption{Overhead - Postgres - 10GB}
%       \label{fig:cap-tpch-post-10gb}
%     \end{subfigure}
%     \begin{subfigure}{0.31\linewidth}
%       \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_10GB_capture.pdf}
%       \caption{Overhead - MonetDB - 10GB}
%       \label{fig:monetdb-tpch-overhead-10gb}
%     \end{subfigure}
%     \caption{Runtime and overhead of queries instrumented to capture provenance sketches relative to queries without instrumentation for TPC-H queries.}
%     \label{fig-exp-runtimes-usage}
%   \end{minipage}
%   %%%%%%%%%%%%%%%%%%%% CAPTURE
%   \begin{minipage}{1.0\linewidth}
%         \includegraphics[width=1\linewidth,trim=0pt 0pt 0 0pt, clip]{figs/binary_search/selectivity_1g_stack.pdf}
%       	\caption{Selectivity TPC-H 1GB}
%       	\label{fig:sel-tpch-1gb}
%     \end{minipage}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/exp_figs_short2.tex <==
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
  \centering
   %%%%%%%%%%%%%%%%%%%% PS legend
  \begin{minipage}{1.0\linewidth}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/pslegend.pdf}
  \end{minipage}

   %%%%%%%%%%%%%%%%%%%% Postgres runtime + overhead
  \begin{minipage}[t]{1.0\linewidth}
    \begin{subfigure}{0.49\linewidth}
      \centering
      \includegraphics[height=3cm,trim=25pt 25pt 0 24pt, clip]{figs/binary_search/version1/post_tpch_1GB_runtime.pdf}
      \trimfigspace
      \caption{Postgres Use - 1GB (BS)}
      \label{fig:tpch-post-1gb}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
      \centering
      \includegraphics[height=3cm,trim=25pt 25pt 0 24pt, clip]{figs/binary_search/version1/post_tpch_1GB_capture.pdf}
      \trimfigspace
      \caption{Postgres Capture - 1GB}
      \label{fig:cap-tpch-post-1gb}
    \end{subfigure}
  \end{minipage}

 %%%%%%%%%%%%%%%%%%%% postgres overhead and selectivities
  \begin{minipage}{1.0\linewidth}
    \begin{subfigure}{0.235\linewidth}
     \begin{adjustbox}{minipage=\linewidth,scale=1.05}
      \centering
      \includegraphics[height=2.3cm,width=1\linewidth,trim=25pt 25pt 0pt 25pt, clip]{figs/realdb/cs/post_realdb_runtime.pdf}
      \trimfigspace \trimfigspace
            \end{adjustbox}
      \caption{Crimes and SOF - Use (OR)}
      \label{fig:realdb-use}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
    \begin{adjustbox}{minipage=\linewidth,scale=1.05}
      \centering
      \includegraphics[height=2.3cm,width=1\linewidth,trim=25pt 26pt 0pt 21pt, clip]{figs/realdb/cs/post_realdb_capture.pdf}
      \trimfigspace \trimfigspace
             \end{adjustbox}
      \caption{Crimes and SOF - Capture}
      \label{fig:realdb-cap}
    \end{subfigure}
    \begin{subfigure}{0.28\linewidth}
      \begin{adjustbox}{minipage=\linewidth,scale=0.95}
      \includegraphics[height=2.8cm,trim=25pt 32pt 21pt 35pt, clip]{figs/binary_search/version1/post_tpch_10GB_runtime.pdf}
      \trimfigspace \trimfigspace
                \end{adjustbox}
      \caption{Postgres Use - 10GB (BS)}
      \label{fig:tpch-post-10gb}
    \end{subfigure}\hspace{-8pt}
    \begin{subfigure}{0.23\linewidth}
    \begin{adjustbox}{minipage=\linewidth,scale=0.95}
      \includegraphics[height=2.8cm,trim=32pt 32pt 21pt 20pt, clip]{figs/binary_search/version1/post_tpch_10GB_capture.pdf}
      \trimfigspace \trimfigspace
             \end{adjustbox}
      \caption{Postgres Capture - 10GB}
      \label{fig:cap-tpch-post-10gb}
    \end{subfigure}
  \end{minipage}

   %%%%%%%%%%%%%%%%%%%% monetdb runtime + overhead
  \begin{minipage}{1.0\linewidth}
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=1\linewidth,trim=20pt 25pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_1GB_runtime.pdf}
      \trimfigspace[-5mm]
      \caption{MonetDB Use - 1GB (OR)}
      \label{fig:monetdb-tpch-1gb}
    \end{subfigure}
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=1\linewidth,trim=20pt 25pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_10GB_runtime.pdf}
      \trimfigspace[-5mm]
      \caption{MonetDB Use - 10GB (OR)}
      \label{fig:monetdb-tpch-10gb}
    \end{subfigure}
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=1\linewidth,trim=20pt 25pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_1GB_capture.pdf}
      \trimfigspace[-5mm]
      \caption{MonetDB Capture - 1GB}
      \label{fig:monetdb-tpch-overhead-1gb}
    \end{subfigure}
    \begin{subfigure}{0.245\linewidth}
      \includegraphics[width=1\linewidth,trim=20pt 25pt 0 0pt, clip]{figs/monetdb/monetdb_tpch_10GB_capture.pdf}
      \trimfigspace[-5mm]
      \caption{MonetDB Capture - 10GB}
      \label{fig:monetdb-tpch-overhead-10gb}
    \end{subfigure}
    \trimfigspace
    \caption{Performance of provenance sketch capture and use for Crimes, SOF and TPC-H queries.}
    \label{fig-exp-runtimes-usage}
  \end{minipage}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/overview.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Overview}
\label{sec:overview}

